The first identification of Lyman $\alpha$ Changing-look Quasars at high-redshift in DESI

We present two cases of Ly$\alpha$ changing-look (CL) quasars (J1306 and J1512) along with two additional candidates (J1511 and J1602), all discovered serendipitously at $z >2$ through the Dark Energy Spectroscopic Instrument (DESI) and the Sloan Digital Sky Survey (SDSS). It is the first time to capture CL events in Ly$\alpha$ at high redshift, which is crucial for understanding underlying mechanisms driving the CL phenomenon and the evolution of high-redshift quasars and galaxies. The variability of all four sources is confirmed by the significant change of amplitude in the $r$ band ($|r_{\rm DESI}-r_{\rm SDSS}| >0.5 \ \rm mag$). We find that the accretion rate in the dim state for these CL objects corresponds to a relatively low value ($\mathscr{\dot M} \approx 2\times10^{-3}$), which suggests that the inner region of the accretion disk might be in transition between the Advection Dominated Accretion Flow ($\mathscr{\dot M}<10^{-3}\sim 10^{-2}$) and the canonical accretion disk (optically thick, geometrically thin). However, unlike in C {\sc iv} CL quasars in which broad Ly$\alpha$ remained, the broad C {\sc iv} may still persist after a CL event occurs in Ly$\alpha$, making the physical origin of the CL and ionization mechanism event more puzzling and interesting.

==> table.tex <==
\begin{deluxetable*}{ccccccccc}
\tablecolumns{9}
\tabletypesize{\footnotesize}
\tabcaption{\centering  The information of four Ly$\alpha$ CL AGN
\label{tab2}}
\colnumbers
\tablehead{
\colhead{Object Name} &
\colhead{Observation} &
\colhead{R.A.} &
\colhead{Dec.} &
\colhead{$z$} &
\colhead{mag($g$,$r$,$z$),exp\_time(MJD)} &
\colhead{MJD} &
\colhead{$\log(M_{\bullet}/M_{\odot})$} &
\colhead{FWHM} &
\colhead{state} 
}
\startdata
J151122.19+291321.8 & SDSS & 227.8425  & 29.2227 & 2.211 & 
g=22.04, r=22.10, z=21.34 57714.666 \\
\nodata             & DESI & 227.8425  & 29.2227 & 2.214  & u=21.576, g=21.179,r=21.250,i=21.215,z=21.004 &53081\\
\hline
J151205.89+374627.7 & SDSS & 228.0245  & 37.7744 & 2.221 &
g=22.50, r=22.56, z=21.83   57581.74\\
\nodata             & DESI & 228.0245  & 37.7743 & 2.222 &u=23.142, g=22.160, r=21.988, i=21.956, z=21.647 52704\\
\hline
J160222.63+174905.5 & SDSS & 240.5943  & 17.8182 & 2.738 & 
g=21.62, r=21.32, z=21.42   57858.939 \\
\nodata             & DESI & 240.5943  & 17.8182 & 2.733 & u=23.91, g=22.11, r=21.89, i=22.10, z=21.96  53148 \\
\hline
J130643.24+561842.1 & SDSS & 196.6802  & 56.3117 & 2.638 & u=22.69, g=21.78, r=21.55, i=21.78, z=21.42.  52708\\ 
\nodata             & DESI & 196.6803  & 56.3117 & 2.633 & 
g=22.63, r=22.74, z=22.71   57702.75 \\
\enddata
\tablecomments{Columns: (1) BEL name, (2) BEL wavelength, (3) BEL integration windows,  (4) left background windows, (5) right background windows, (6) number of the CL AGN founded in DESI, (7) number of the CL candidates founded in DESI, (8)  physical mechanism of the BEL.
}
\end{deluxetable*}

